Robust Multi-agent Communication Based on Decentralization-Oriented Adversarial Training

In typical multi-agent reinforcement learning (MARL) problems, communication is important for agents to share information and make the right decisions. However, due to the complexity of training multi-agent communication, existing methods often fall into the dilemma of local optimization, which leads to the concentration of communication in a limited number of channels and presents an unbalanced structure. Such unbalanced communication policy are vulnerable to abnormal conditions, where the damage of critical communication channels can trigger the crash of the entire system. Inspired by decentralization theory in sociology, we propose DMAC, which enhances the robustness of multi-agent communication policies by retraining them into decentralized patterns. Specifically, we train an adversary DMAC\_Adv which can dynamically identify and mask the critical communication channels, and then apply the adversarial samples generated by DMAC\_Adv to the adversarial learning of the communication policy to force the policy in exploring other potential communication schemes and transition to a decentralized structure. As a training method to improve robustness, DMAC can be fused with any learnable communication policy algorithm. The experimental results in two communication policies and four multi-agent tasks demonstrate that DMAC achieves higher improvement on robustness and performance of communication policy compared with two state-of-the-art and commonly-used baselines. Also, the results demonstrate that DMAC can achieve decentralized communication structure with acceptable communication cost.

==> sec/4_approach.tex <==
% \section{{\tooladv}}
% \label{sec:adv}

% % \subsection{{\tool}}
% % \label{subsec:overview}
% % The goal of {\tool} is to \yawen{learn a robust communication policy}\rev{optimize the learnable-based communication policy, thereby increasing robustness} against various attacks.
% % As shown in Figure \ref{fig:overview}, there is an existing communication policy model $CP$ being trained, which takes environmental information as input and outputs a benign communication policy. {\tool} builds an adversary as a component, called {\tooladv}, which also takes environmental information as input and outputs a cutting policy to perturb communication connections between certain agents. As introduced in Section \ref{sec:intro}, inspired by decentralization, {\tool} can identify and cut off the critical communication connections. As we can see, after the perturbation, the original centralized communication policy is destroyed and a decentralized perturbed communication policy is formed. Then the agents make subsequent decisions based on the perturbed communication policy and continues to train $CP$ based on adversarial training.
% % \yawen{comment}
% % 上述内容是不是应该放到问题定义里面去？fig 2应该在Sec 3，Sec 4直接介绍Fig 3了？需要想明白问题定义里面都要介绍哪些内容
% % 内容表述的也不是很清楚，对于target来说，不知道pi跟cm的区别，对于RMAC，不知道整体的工作机制，以及为什么就能decentralization

% \xuyan{The key to achieve decentralization is to perturb critical communication connections in the adversarial learning process of the communication policy, forcing it to adjust its policy to tend to decentralization. Based on this, we propose {\tooladv}, which is used as a component of {\tool} for identifying and cutting off the critical communication connections.}
% % \rev{{\tooladv} aims to identify and cut off critical communication connections between the multiple agents, \xuyan{so that in order to influence the target agents’ reward.}}
% % so that the multi-agent system can not complete its task.
% \yawen{comment}
% % so that the multi-agent system can not complete its task.?你这是不是还是从攻击角度说的？
% % \rev{At the same time,} 
% % \xuyan{In addition, we design the input of {\tooladv} and reconstruct the reward function which will be detailed in the following.}
% % As for the second challenge, in order to balance robustness and performance, {\tooladv}  minimizes the number of cut communication connections. 
% \yawen{comment}
% % 这段描述也没啥信息量。这个embedding的部分感觉应该算在RMAC_Adv里面介绍，但是叫input也不是很好



% \subsection{Input of {\tooladv}}
% \subsection{Environmental Information Awareness?}
% \label{subsec:input}
% \xuyan{Using observations to determine communication policy is a common setting, however, this setting lacks a description of the relationships between agents and the team structure \cite{MaWWXWLX024}, making it difficult to mine critical communication connections.}
% To better represent the state of each agent and the relationship between agents, we not only use the observations of the agents as input, but also abstract the relationship between agents and their neighbors. 
% \yawen{comment}
% % 这块为了更好表示所做的设计，前面也没有任何铺垫，或是能对应上某个挑战？

% \xuyan{Firstly, we can obtain the observation of the each agent $\{o_1,...,o_n\}$ from the environment.}
% \xuyan{Then, we get the representation of each agent $\{e_1,...,e_n\}$ (called \textit{embedding representation}) based on the agent itself and its neighbors. \rev{Evaluation of the necessity of embedding representation is given in the Appendix \ref{sec:app}.}} 
% % As described in Section \ref{subsec:model}, the target agents team can be modeled as an undirected graph. 
% We model the target agents team and interactions between teammates as an undirected graph, with each agent represented as a vertex. The state information and cooperative relationships of the target agents are effectively represented by the graph's structure, the properties of the vertices, and the weights of the edges. Each vertex holds a set of properties for the corresponding agent, such as, location, speed, health, and so on. The edges between vertices and their weights are the interactions and situations between two agents. The weight of an edge is determined by the distance between two agents, as obtained from the environment, indicating the degree to which the two agents can interact with each other. 
% \yawen{comment}
% % 不同环境都是用的distance吗
% % As we can see in Figure \ref{fig:adv}a, {\tooladv} can obtain the observation of the each agent $\{o_1,...,o_n\}$ and the embedding representation of each agent $\{e_1,...,e_n\}$ from the environment.
% \yawen{comment}
% % embedding representation指的是图表示的结果吗？前面也没铺垫突然出来这个词很迷惑
% % 另外考不考虑增加实验证明这个设计的必要性，可以加到appendix
% The embedding representation is calculated as follows:

% % \xuyan{comment} %直接复制了issta的内容，需要换说法
% First, {\tool} initializes the embedding representation of each vertex based on its own attribute. Then, {\tool} aggregates the information from neighboring vertices using a weight-based aggregation function. For a vertex $v$, $\mathcal{N}(v)$ is the neighbor vertices of $v$ and $e^{k}_{v}$ is the embedding representation of vertex $v$ after the $k$-th iteration.
% $w(u,v)$ is the weight of the edge between vertices $u$ and $v$, quantifying the interaction between the two agents and how they interact. We represent the weight by the distance between two agents, obtained from the environment, which indicates the extent to which the agents can interact.
% Then the embedding of $v$ at $(k+1)$-th iteration $e^{k+1}_{v}$ is the sum of $e^{k}_{v}$ and the weighted and averaged neighbor embedding, which is specified as follows:
% \begin{equation}
% \label{equ:aggregate}
%     e^{k+1}_{v} \leftarrow Sum(e^{k}_{v}, Mean({\frac{1}{w(u,v)} * e^{k}_{u} ), u \in \mathcal{N}(v) }).
% \end{equation}
% In this way, we can obtain the embedding representation of each vertex as $e_{v}$.

% As shown in Figure \ref{fig:adv}b, we concatenate the observation and embedding representation to get new representation $\{g_1,...,g_n\}$, where $g_i = o_i \oplus e_i$. 
% % \yawen{comment}
% % \odot前面用过了，有别的含义了
% Finally, we send $g_i$ and $g_j$ to the cutting agent for subsequent decision making about whether to sever the communication connection between agents $i$ and $j$. 
% % Then, we merge the representation of two agents $i,j$ and input the feature into the BiLSTM \cite{ZhangZHY15} model:
% % \begin{equation}
% % \label{equ:lstm}
% %     h_{i,j} = BiLSTM(g_i, g_j).
% % \end{equation}
% % BiLSTM can effectively eliminate the effects of different order of inputs (agents). Based on this, we obtain the agent-pair embedding $h_{i,j}$ for agent $i$ and agent $j$.
% % \yawen{comment}
% % merge是个啥操作。为啥BiLSTM可以消除影响。实际上我们是对每个i和j对进行了表示，然后cutting agent拿这个做输入，输出这个对是否断开？

% \subsection{Architecture of {\tooladv}} 
% {\tooladv} consists of two networks: the policy network of cutting agents $\pi^c$ and the critic network $C$. Specifically, the network $\pi^c$ learns the policy of cutting agents, taking the set $\{g_{1},...,g_{n}\}$ as input and outputting the cutting actions $a^c_{i,j}$, where $i$ and $j$ represent two agents. The critic network $C$ is designed to evaluate the joint actions of all cutting agents from a global perspective.

% Following value-based CTDE, we evaluate the value of cutting actions while learning $\pi^c$. First, we train $\pi^c$ to learn individual value function $Q(a^c_{i,j}, [g_i,g_j])$ for each cutting agent, which assesses the individual policy. This value function represents the benefit of taking action $a^c_{i,j}$ given the representation $[g_i,g_j]$. Second, $C$ learns the centralized value function $Q_{tot}(a^c_{i,j}, [g_i,g_j])$ to evaluate the collective policy, providing an estimate of the adversary reward $\hat{r}$.

% To maximize both individual and total values simultaneously, this can be achieved by adhering to the Individual-Global-MAX (IGM) principle \cite{HongJT22}:

% % \begin{equation}
% % \label{equ:igm}
% % \begin{aligned}
% %     & \arg \max_{a^c \in \mathcal{A}^c} Q_{tot} (h, a^c)= \\
% %     & \left<\arg \max_{a^c_{1,2}} Q(h_{1,2}, a^c_{1,2}), \dots, \arg \max_{a^c_{n-1,n}} Q(h_{n-1,n}, a^c_{n-1,n}) \right>
% % \end{aligned}
% % \end{equation}


% \begin{equation}
% \label{equ:igm}
% \arg \max_{a^c \in \mathcal{A}^c} Q_{tot} (h, a^c)= \left( 
% \begin{aligned}
%   &\arg \max_{a^c_{1,2}} Q([g_1,g_2], a^c_{1,2}) \\
%   &\dots \\
%   &\arg \max_{a^c_{n-1,n}} Q([g_{n-1},g_n], a^c_{n-1,n})
% \end{aligned}
% \right)
% \end{equation}

% % \begin{equation}
% %     \label{equation:igm}
% %     \begin{aligned}
% %     & \arg\max_{a^m\in \mathcal{A}^{m}} Q_{tot}(o, a^m; \omega) = \\
% %     & \left< \arg\max_{a^m_1} Q_1(o_1, a^m_1; \theta), ..., \arg\max_{a^m_n} Q_n(o_n, a^m_n; \theta) \right>.
% %     \end{aligned}
% % \end{equation}

% Specifically, in {\tooladv}, we constrain the weights $\omega$ of the critic network $C$ to be non-negative to ensure adherence to the Equation \ref{equ:igm}, which can be defined as follows:
% \begin{equation}
% \label{equ:weights}
% \begin{aligned}
%     &Q_{tot}(g, a^c; \omega) = \omega (Q([g_i,g_j], a^c_{i,j})), \forall{i,j} \in \{1, \dots, n\}, \\ 
%     &i \neq j; \omega \geq 0.
% \end{aligned}
% \end{equation}
% Equation \ref{equ:weights} can be replaced with other implements such as VDN \cite{SunehagLGCZJLSL18}, OPLEX \cite{WangRLYZ21}, and QTRAN \cite{SonKKHY19}. \xuyan{comment} %必要时可删除

% Finally, we use TD losses \cite{HausknechtS15} as the loss function of {\tooladv} for iterative optimization of $\pi^c$ and $C$, to minimize the error gap between the expected value and the estimate value $Q_{tot}(g, a^c)$.
% \begin{equation}
%     \mathcal{L} = \arg \min \mathbb{E} [(y_{tot}-Q_{tot}(g,a^c))^2]
% \end{equation}
% where $y_{tot} = \hat{r} + \gamma \max_{\Tilde{a}^c} \Tilde{Q}_{tot} (\Tilde{g}, \Tilde{a}^c)$, which denotes the expected value. $\hat{r}$ is the adversary reward introduced in Equation \ref{equ:obj} and $\Tilde{Q}_{tot} (\Tilde{g}, \Tilde{a}^c)$ is calculated for the next time step by the stale network. Since Equation \ref{equ:igm} holds, we can perform the maximization of $Q_{tot}$. Previous work \cite{LiuZC23} has demonstrated the feasibility and stability of implementing updates in this manner.
% Algorithm \ref{alg:adv} briefly presents the training process of {\tooladv}.



% \begin{algorithm}
% \caption{The training algorithm of {\tooladv}}
% \label{alg:adv}
% \begin{algorithmic}[1]
% \State \textbf{Input:} The policy $\pi$ of target agents, the observations $\{o_1, \dots, o_n\}$, the embedding of each agent $\{g_{1}, \dots, g_{n}\}$.
% \State \textbf{Output:} The policy $\pi^c$ of cutting agents
% \State \textbf{Initialization:} The networks of $\pi^c$ and $C$ 
% % \State $x \gets 0$  \Comment{Initialize sum t}
% \For{$each$ $training$ $batch$}
%     % \State $x \gets x + a_i$
%     \State Get joint cutting action and values from $\pi^c$:
%     \State $\{a_{1,2}^c, \dots, \}, \{Q(h_{1,2},a_{1,2}^c), \dots, \} = \pi^c(h_{1,2}, \dots, )$
%     \State Get the number of attacks $r^c$
%     \State Get the final observations:
%     \State $\{\hat{o}_1, \dots, \hat{o}_n\} = \{o_1, \dots, o_n\} \odot \{a_{1,2}^c, \dots, a_{n-1,n}^c\} $
%     \State Get joint action from $\pi$
%     \State $\{a_1, \dots, a_n\} = \pi(\hat{o}_1, \dots, \hat{o}_n)$
%     \State Execute joint action %of target agents
%     and get reward $r$ from env
%     \State Calculate the global value $Q_{tot}$ using network $C$
%     \State Update $\pi_c$ and $C$ by the TD loss with $r$, $r^c$ and $Q_{tot}$
% \EndFor
% \State \textbf{return} $\pi_c, C$
% \end{algorithmic}
% \end{algorithm}









==> table/table_ablation.tex <==
\begin{table}[h]
\renewcommand\arraystretch{1.1}
\centering
\caption{The win rate of the target MAS with two communication policies under attack in two settings. $ER$ means the \textit{embedding representation}.}
\label{tab:abl1}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{c|cccc|cccc} \toprule 
\textbf{Attack Method} & \multicolumn{4}{c|}{\textbf{Learned Adaptive Attack}} & \multicolumn{4}{c}{\textbf{Heuristic Attack}} \\ \midrule
 \diagbox{\textbf{Method}}{\textbf{Env}}& \textbf{SC} &  \textbf{CN} &\textbf{TJ} & \textbf{PP}  & \textbf{SC} &  \textbf{CN} &\textbf{TJ} & \textbf{PP} \\ \midrule 
\textbf{T2MAC+{\tool}}  & \textbf{60.4\%} & \textbf{62.7\%} & \textbf{70.4\%} & \textbf{66.3\%} & \textbf{69.9\%} & \textbf{70.1\%} & \textbf{73.8\%} & \textbf{74.4\%} \\
 \textbf{T2MAC+{\tool}-$ER$}& 49.5\%   & 50.3\%   & 58.2\%   & 48.7\%   & 51.7\%  & 59.4\% & 60.1\% & 54.0\% \\

\hline 
\hline
\textbf{I2C+{\tool}} & \textbf{58.3\%} & \textbf{59.9\%} & \textbf{67.3\%} & \textbf{62.5\%} & \textbf{66.4\%} & \textbf{68.2\%} & \textbf{70.1\%} & \textbf{71.9\%} \\
 \textbf{I2C+{\tool}-$ER$}& 40.6\% & 42.1\% & 51.0\% & 49.8\% & 46.6\% & 52.9\% & 59.9\% & 61.2\% \\


 \bottomrule
\end{tabular}}
\end{table}







\begin{table}[htbp]
\centering
\renewcommand\arraystretch{1.1}
\caption{The win rate of the target MAS with two communication policies in two settings. $ER$ means the \textit{embedding representation}.
% ``Original'' represents the performance of the communication model without optimization.
% \yawen{comment}
% 这个original是不是你就选了一个T2MAC作为例子，是不是T2MAC，I2C都列上啊，要不跟Table 1一样？
}
\label{tab:abl2}
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{c|cccc} \toprule 
 % & \multicolumn{4}{c|}{\textbf{T2MAC}} & \multicolumn{4}{c}{\textbf{I2C}}  \\ \midrule 
\diagbox{Method}{Env}   & \textbf{SC} &  \textbf{CN} &\textbf{TJ} & \textbf{PP}  \\ \midrule 


\textbf{T2MAC+{\tool}} & \textbf{83.7\%} & \textbf{89.5\%} & \textbf{93.8\%} & \textbf{90.7\%}  \\  
\textbf{T2MAC+{\tool}-$ER$} & 83.1\% & 89.0\% & 92.5\% & 89.9\%  \\  
\hline 
\hline

\textbf{I2C+{\tool}} & \textbf{79.4\%} & \textbf{83.6\%} & \textbf{90.4\%} & \textbf{88.1\%} \\

\textbf{I2C+{\tool}-$ER$} & 78.5\% & 82.4\% & 88.7\% & \86.6\%  \\  

 \bottomrule
\end{tabular}}
\end{table}

==> table/table_acc.tex <==
% \begin{table*}[]
% \renewcommand\arraystretch{1.2}
% \centering
% \caption{The win rate of the communication model in four environments under various attack. ``Original'' represents the performance of the communication model without optimization. The lower win rate, the better the attack capability.}
% \label{tab:rq3}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l|cccc|cccc} \toprule 
%  & \multicolumn{4}{c|}{\textbf{T2MAC}} & \multicolumn{4}{c}{\textbf{I2C}}  \\ \midrule 
% \diagbox{\textbf{Win Rate}}{\textbf{\%Attack}}     & SC      & CN     & TJ     & PP     & SC     & CN     & TJ     & PP     \\ \midrule 
% \textbf{Original}     & 81.2\% $\mid$ 0\%   & 87.4\% $\mid$ 0\% & 91.7\% $\mid$ 0\% & 88.6\% $\mid$ 0\% & 76.9\% $\mid$ 0\% & 80.1\% $\mid$ 0\% & 85.2\% $\mid$ 0\% & 82.4\% $\mid$ 0\% \\
% % \textbf{Random}     & 57.2\%  & 61.4\% & 63.6\% & 61.7\% & 51.8\% & 55.4\% & 59.3\% & 57.2\% \\
% \textbf{Learned Adaptive Attack}  & 27.8\% $\mid$ 22.2\%  & 30.1\% $\mid$ 28.6\% & 45.8\% $\mid$ 20\% & 37.9\% $\mid$ 25\% & 22.4\% $\mid$ 22.2\% & 24.3\% $\mid$ 28.6\% & 37.7\% $\mid$ 20\% & 32.5\% $\mid$ 25\% \\
% \textbf{Heuristic Attack} & 32.1\% $\mid$ 22.2\% & 37.7\% $\mid$ 28.6\% & 43.6\% $\mid$ 20\% & 39.1\% $\mid$ 25\% & 27.4\% $\mid$ 22.2\% & 30.8\% $\mid$ 28.6\%  & 38.2\% $\mid$ 20\% & 35.7\% $\mid$ 25\% \\

% \textbf{{\tooladv}} & \textbf{16.6\% $\mid$ 8.9\%} & \textbf{19.9\% $\mid$ 10.5\%} & \textbf{34.9\% $\mid$ 8.7\%} & \textbf{26.9\% $\mid$ 9.3\%} & \textbf{12.3\% $\mid$ 7.8\%} & \textbf{14.9\% $\mid$ 7.6\%} & \textbf{30.1\% $\mid$ 7.8\%} & \textbf{22.4\% $\mid$ 8.2\%} \\
%  \bottomrule
% \end{tabular}}
% \end{table*}


\begin{table}[tbp]
\renewcommand\arraystretch{1.1}
\centering
\caption{The win rate of the target MAS with two communication policies in four environments under various attack. The table shows three different ways to identify and attack communication connections: reward-based, random, and {\tool}. The lower the win rate, the higher the identification accuracy of critical communication connections.}
\label{tab:rq3}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{c|c|cccc} \toprule 
% & & \multicolumn{4}{c|}{\textbf{T2MAC}} & \multicolumn{4}{c}{\textbf{I2C}}  \\ \midrule 
\textbf{$CP$} &  \textbf{Attack Method}  & \textbf{SC} &  \textbf{CN} &\textbf{TJ} & \textbf{PP}   \\ \midrule 
% \textbf{Original}     & 81.2\%    & 87.4\%  & 91.7\%  & 88.6\%  & 76.9\%  & 80.1\%  & 85.2\%  & 82.4\%  \\
% \textbf{Random}     & 57.2\%  & 61.4\% & 63.6\% & 61.7\% & 51.8\% & 55.4\% & 59.3\% & 57.2\% \\

\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{T2MAC}}} & \textbf{Reward-Based Attack}  & 37.8\%   & 40.1\%  & 55.8\%  & 47.9\%    \\
&\textbf{Random Attack} & 42.1\%  & 47.7\%  & 53.6\%  & 49.1\%    \\

&\textbf{{\tooladv}} & \textbf{16.6\% } & \textbf{19.9\% } & \textbf{34.9\% } & \textbf{26.9\%}  \\ \hline
\hline

\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{I2C}}} & \textbf{Reward-Based Attack}   & 32.4\%  & 34.3\%  & 47.7\%  & 42.5\%  \\
& \textbf{Random Attack}  & 37.4\%  & 40.8\%   & 48.2\%  & 45.7\%  \\

& \textbf{{\tooladv}} & \textbf{12.3\% } & \textbf{14.9\% } & \textbf{30.1\% } & \textbf{22.4\% } \\

 \bottomrule
\end{tabular}}
\end{table}





